Beating 1-1/e for Ordered Prophets

Hill and Kertz studied the prophet inequality on iid distributions [The Annals of Probability 1982]. They proved a theoretical bound of $1-\frac{1}{e}$ on the approximation factor of their algorithm. They conjectured that the best approximation factor for arbitrarily large n is $\frac{1}{1+1/e} \approx 0.731$. This conjecture remained open prior to this paper for over 30 years. In this paper we present a threshold-based algorithm for the prophet inequality with n iid distributions. Using a nontrivial and novel approach we show that our algorithm is a 0.738-approximation algorithm. By beating the bound of $\frac{1}{1+1/e}$, this refutes the conjecture of Hill and Kertz. Moreover, we generalize our results to non-iid distributions and discuss its applications in mechanism design.

==> hardness.tex <==
\begin{proofof}{Theorem \ref{theorem:hardness}}
	Pick arbitrary numbers $m$ and $\epsilon$. Suppose we have $2m$ distribution. Each of the first $m$ distributions gives $1$ with probability $1$. Each of the last $m$ distributions gives $0$ with probability $(1-\epsilon)^{1/m}$ and $\frac{1}{\epsilon}$ otherwise. Notice that with probability $\Big((1-\epsilon)^{1/m}\Big)^m = 1-\epsilon$ all of the last $m$ items are $0$ and with probability $\epsilon$ at least one of the last $m$ items is $\frac 1 {\epsilon}$. Hence in expectation the optimum takes $$1\times(1-\epsilon)+\epsilon\times\frac 1 {\epsilon}=2-\epsilon.$$ While any online algorithm takes at most $\max(1,\epsilon\times\frac 1 {\epsilon})=1.$ Therefore, the approximation factor of any online algorithm is upper-bounded by $$\frac{1}{2-\epsilon} =\frac{2+\epsilon}{4-\epsilon^2}\leq \frac {2+\epsilon}{4}\leq  0.5 + \epsilon.$$
\end{proofof}

==> old_notes/best_order.tex <==
The best order problem is the problem of finding how good one can achieve on the best order of the input sequence. We approach this problem by first creating a new order for the items in $A$ and then giving an algorithm that works well on this new order. The order we create is in fact a uniform grouping of the items in $A$ which in a big picture makes the input look like an \textit{i.i.d.} sequence. Surprisingly, an algorithm similar to our algorithm for the \textit{i.i.d.} setting works quite well on this particular sort of orders.

\begin{theorem} \label{theorem:best_order}
	For a given sequence $A$ of distributions with frequency at least $(1/\epsilon)^2$, there exists an algorithm that has a $(1-\epsilon)^2 0.74$-competitive ratio on the best order of $A$.
\end{theorem}

%\todo{somewhere here mention that we have $f_i(A)\geq (1/\epsilon)^2$.}

We will later explain our methods for grouping and picking policy in detail. But let us begin with the following lemma, which states discarding a small fraction of distributions does not hurt the optimum solution largely.

\begin{lemma} \label{lemma:throw_away}
	For a given sequence of distributions $A$ and a subsequence $A'$ of it with $f_i(A')\geq (1-\epsilon)f_i(A)$ for every $1\leq i \leq m$, we have $OPT(A')\geq (1-\epsilon)OPT(A)$.
\end{lemma}

\begin{proof}
	Let $X$ and $X'$ be sequences of random variables that are drawn from $A$ and $A'$ respectively. Since $A'$ is a subsequence of $A$ there exists a mapping between every $X'_j$ and some $X_{r_j}$ which has the same distribution type as $X'_j$. We can observe that the probability of $X'_j$ being the maximum in $X'$ is not less than the probability of $X_{r_j}$ being the maximum in $X$. This is because there are some other distributions in $A$ in addition to all distributions in $A'$ that may decrease the chance of $X_{r_j}$ being the maximum. The following corollary is a generalization of this observation.
	
	\begin{corollary} \label{corollary:throw_away}
	$\forall t\in \mathbb{R^+}: Pr[X'_j\geq t | X'_j=\max\{X'_i\}] \geq Pr[X_{r_j} \geq t|X_{r_j}=\max\{X_i\}]$.
	\end{corollary}
	
	Now from the definition of $OPT$ we have:
	\begin{align*}
		OPT(A') &= E[\max\{X'_i\}] & \\ &= \sum_{j=1}^{|X'|} E[X'_j|X'_j=\max\{X'_i\}] \\
		&= \sum_{j=1}^{|X'|} \int_{0}^{\infty} Pr[X'_j>t|X'_j=\max\{X'_i\}] dt \\
		&\geq \sum_{j=1}^{|X'|} \int_{0}^{\infty} Pr[X_{r_j}>t|X_{r_j}=\max\{X_i\}] dt &Corollary \ref{corollary:throw_away} \\
		&\geq (1-\epsilon)\sum_{j=1}^{|X|} \int_{0}^{\infty} Pr[X_j>t|X_j=\max\{X_i\}] dt & f_i(A')\geq (1-\epsilon)f_i(A)\\
		&= (1-\epsilon)OPT(A) \enspace .\\
	\end{align*}
	
\end{proof}

Lemma \ref{lemma:throw_away} states that removing a small fraction of distributions does not hurt the optimum solution significantly. We use this fact to build a new order $B$ of the distributions in $A$ that has an optimal solution comparable to the one for $A$. We then give a competitive algorithm that works well on $B$. As a result, our algorithm also gives a lower bound for the best ordering of distributions in $A$.

Sequence $B$ is in fact composed of $l=1/\epsilon$ groups $G_1,\ldots,G_l$ each of which having the same set of distributions. In other words, we make a new sequence $B$ consisting of $l$ consecutive chunks. Each of these chunks has an arbitrary order but the same number of distributions of every type. Therefore $f_k(G_i)=f_k(G_j)$ for every $1\leq k\leq m$ and $1\leq i,j\leq l$. To this end, we need every $f_i(B)$ to be divisible to $l$. This can be done by omitting a small fraction \footnote{At most $l-1$ out of $f_i(A)$ instances.} of the distributions of every type in $A$, meaning that we treat them as though they do not exist in sequence $B$.

\begin{lemma} \label{lemma:frequencies_remain_good}
	For every $1\leq i\leq l$, if $f_i(A)>l^2$ then $f_i(B)>(1-\epsilon)f_i(A)$.
\end{lemma}
\begin{proof}
	For every particular type $T_i$ we have $f_i(A)$ instances of the distributions of this type in $A$. In order to reach a number of distributions divisible to $l$ we need to discard at most $l-1$ instances. Therefore,
	$$f_i(B)\geq f_i(A)-(l-1) > f_i(A)-\frac{f_i(A)}{l} \geq (1-\epsilon)f_i(A)\enspace .$$
\end{proof}

Although not improving the competitive ratio, omitting these items simplifies our analysis. Lemma \ref{lemma:frequencies_remain_good} and Lemma \ref{lemma:throw_away} imply that the optimum solution to $B$ remains within a range of $\epsilon$ from the optimum solution to $A$, \todo{i.e.} $OPT(B)\geq (1-\epsilon)OPT(A)$.

We now give an algorithm to find a competitive solution in the online scenario of $B$. To make a better understanding of the algorithm we first define a new sequence of distributions $C$ of length $l$ such that every $C_i$ is the distribution of the maximum value in group $i$. In other words every $C_i$, $1\leq i\leq l$, is defined as $C_i:=\max_{B_j\in G_i}\{X^B_j\}$ where $X^B_j$ indicates a random variable drawn from $B_j$. Note that with this definition all $C_i$'s are \textit{i.i.d.} because we spread the distributions of every type $T_r$, $1\leq r\leq m$, uniformly among $G_i$'s.

\begin{corollary} \label{corollary:C_is_iid}
	The distributions in $C$ are \textit{i.i.d.} .
\end{corollary}

Moreover, considering that the distribution of maximum value in $C$ is equal to the one for $B$, there is an equality between the optimum solution of $B$ and the optimum solution of $C$.

\begin{corollary} \label{corollary:OPT_B=OPT_C}
	$OPT(B)=OPT(C)$.
\end{corollary}

According to Corollary \ref{corollary:C_is_iid} and Theorem \ref{theorem:main}, there exists a sequence of thresholds $\tau_1,\ldots,\tau_l$ for $C$ that gives a solution with 0.74-competitive ratio such that the probability of each \todo{item} $i$ being picked is almost equal to $1/l$.
\todo{The previous sentences need to be rewritten in a more precise way after \ref{theorem:main} is done.}
Using these thresholds we will explain how our algorithm works on sequence $B$. Beginning from $B_1$, the algorithm picks the first item $B_j$ that has a value above the threshold $\tau_{s(j)}$, where $s(j)$ is the index of the group that $B_j$ belongs to. In the following $ALG$ refers to the solution of our algorithms in the online scenario. In particular, $ALG(B)$ and $ALG(C)$ refer to the solution of our algorithms for $B$ and $C$ respectively.

\begin{algorithm} \label{best_order_algorithm}
	\caption{Best Order}
	\textbf{Input: A sequence $A=\langle A_1, \ldots, A_n\rangle$ of distributions generated from a set of distribution types $T=\{T_1,\ldots,T_m\}$, such that $f_i(A)\geq (1/\epsilon)^2$ for every $1\leq i\leq m$.}
	%	\textbf{Output:}
	
	\textbf{Ordering}	
	\begin{algorithmic}[1]
		\scriptsize
		\STATE $l= 1/\epsilon$
		\STATE $B =$ A largest subset of $A$ that can uniformly be partitioned into $l$ groups $G_1,\ldots,G_l$. %, $s.t.$ $f_i(B)\geq (1-\epsilon)f_i(A)$.
		\COMMENT{The remaining distributions in $A$ are treated as though they do not exists.}
	\end{algorithmic}
	
	\textbf{Picking Policy for $B$:}
	\begin{algorithmic}[1]
		\scriptsize
		\STATE $s(j) = $ The index of the group containing $B_j$.
		\STATE $C =$ A sequence of \textit{i.i.d.} distributions, defined as $C_i:=\max_{B_j\in G_i} \{X^B_j\}$.
		\STATE Use \todo{ALG \textit{i.i.d.}} to find thresholds $\tau_1,\ldots,\tau_l$ for $C$.
		\STATE Pick the first item $j$ of $B$ for which $X^B_j\geq \tau_{s(j)}$.		
	\end{algorithmic}
\end{algorithm}

\begin{lemma} \label{lemma:ALG_B>=(1-eps)ALG_C}
	$ALG(B) \geq (1-\epsilon)ALG(C)$.
\end{lemma}

\begin{proof}
	Let $X_B$ be a random variable for the output of our algorithm on $B$, and $X_C$ be a random variable for the output of our algorithm on the \textit{i.i.d.} sequence $C$. We use $X^B_j$ and $X^C_i$ as random variables denoting the value of $j$'th item in $B$ and $i$'th item in $C$ respectively. Every item in $B$ belongs to one of group among $G_1,\ldots,G_l$. Regarding these notations, our algorithm picks the first item $B_j$ for which $X^B_j>\tau_{s(j)}$. Moreover, in the following $p_i$ denotes the probability of our algorithm picking no item from the first $i-1$ items, i.e. $p_i := \prod_{r<i} Pr[X^C_r<\tau_r]$.
	
	\begin{corollary} \label{corollary:p_i}
		$\prod_{j:s(j)<i}Pr[X^B_j<\tau_{s(j)}]=\prod_{r<i}Pr[X^C_r<\tau_r]=p_i$ \enspace .
	\end{corollary}
	
	\begin{align*}
 		ALG(B) &= E[X_B] & \\
		&= \sum_{j} E[X^B_j|\textit{j'th item is picked}] \\
		&= \sum_{j}\int_{\tau_{s(j)}}^{\infty}\bigg(Pr[X^B_j>t]\prod_{k<j}Pr[X^B_k<\tau_{s(k)}]\bigg)dt \\
		&= \sum_{j}\int_{\tau_{s(j)}}^{\infty}\bigg(Pr[X^B_j>t]\prod_{k<j:s(k)=s(j)}Pr[X^B_k<\tau_{s(k)}]\prod_{k:s(k)<s(j)}Pr[X^B_k<\tau_{s(k)}]\bigg)dt \\
		&=
		\sum_{j}\int_{\tau_{s(j)}}^{\infty}\bigg(Pr[X^B_j>t]\prod_{k<j:s(k)=s(j)}Pr[X^B_k<\tau_{s(k)}] p_{s(j)}\bigg)dt & Corollary \ref{corollary:p_i}\\
		&\geq
		\sum_{j}\int_{\tau_{s(j)}}^{\infty}\bigg(Pr[X^B_j>t]\prod_{k:s(k)=s(j)}Pr[X^B_k<\tau_{s(k)}] p_{s(j)}\bigg)dt \\
		&\geq
		\sum_{j}\int_{\tau_{s(j)}}^{\infty}\bigg(Pr[X^B_j>t](1-\epsilon) p_{s(j)}\bigg)dt & Theorem \ref{theorem:main}\\
		&= (1-\epsilon)\sum_{i}\sum_{j:s(j)=i}\int_{\tau_i}^{\infty}\bigg(Pr[X^B_j>t]p_i\bigg) dt \\
		&=
		(1-\epsilon)\sum_{i}\int_{\tau_i}^{\infty}\bigg(\sum_{j:s(j)=i}Pr[X^B_j>t]p_i\bigg) dt\\
		&\geq
		(1-\epsilon)\sum_{i}\int_{\tau_i}^{\infty}\bigg(Pr[\max_{j:s(j)=i} X^B_j>t]p_i\bigg) dt & \textit{Union Bound}\\
		&=
		(1-\epsilon)\sum_{i}\int_{\tau_i}^{\infty}\bigg(Pr[X^C_i>t]p_i\bigg) dt \\
		&=(1-\epsilon)\sum_{i} E[X^C_i|\textit{i'th item is picked}] \\
		&= (1-\epsilon) E[X_C] = (1-\epsilon)ALG(C)	\enspace .
	\end{align*}
\end{proof}

\begin{proof}[Proof of Theorem \ref{theorem:best_order}]
	To wrap up the previous results, we first find a uniformly distributed subsequence of $A$, namely $B$. We then exploit our algorithm for \textit{i.i.d.} sequences to achieve a threshold policy $\tau_{s(j)}$ for every $B_j$. Lemma \ref{lemma:throw_away} gives a lower bound for the offline optimum of $B$, Corollary \ref{corollary:OPT_B=OPT_C} states an equality between the optimum of $B$ and $C$, and Lemma \ref{lemma:ALG_B>=(1-eps)ALG_C} gives a lower bound for the output of our algorithm on $B$. Recall that $ALG(B)$ is the output of our algorithm on some order of $A$, hence the ratio between $ALG(B)$ and $OPT(A)$ gives a lower bound for $c$, where $c$ is the competitiveness on the best order.
	
	\begin{align*}
	c &\geq \frac{ALG(B)}{OPT(A)} & \\
	&\geq \frac{ALG(B)}{\frac{OPT(B)}{1-\epsilon}} & Lemma \ref{corollary:throw_away} \\
	&\geq \frac{ALG(B)}{\frac{OPT(C)}{1-\epsilon}} & Corollary \ref{corollary:OPT_B=OPT_C} \\
	&\geq \frac{(1-\epsilon)ALG(C)}{\frac{OPT(C)}{1-\epsilon}} & Lemma \ref{lemma:ALG_B>=(1-eps)ALG_C} \\
	&\geq (1-\epsilon)^2 0.74 \enspace . & Theorem \ref{theorem:main}
	\end{align*}
\end{proof}

==> old_notes/iid.tex <==
In this section we give a 0.738-approximation algorithm for prophet inequality with iid items. Let us begin with some definitions. Assume that $X_1,\ldots,X_n$ are iid random variables with common distribution function $F$. For simplicity, assume that $F$ is continuous and strictly increasing on a subinterval of $\mathcal{R}^{\geq 0}$. An algorithm based on a sequence of thresholds $\theta_1,\ldots, \theta_n$ is the one that selects the first item $k$ such that $X_k\geq \theta_k$.

Let $\tau$ denote the stopping time of this algorithm, where $\tau$ is $n+1$ when the algorithm picks no item. For simplicity suppose $X_{n+1}$ is a zero random variable. The approximation factor of an algorithm based on $\theta_1\ldots,\theta_n$ is defined as $E[X_\tau]/E[\max X_i]$. This factor captures the ratio between what a player achieves in expectation by acting based on these thresholds and what a prophet achieves in expectation by knowing all $X_i$'s in advance and taking the maximum of them.

In Algorithm \ref{alg:iid} we presents a simple oblivious algorithm for every $n$ and distribution function $F$. Theorem \ref{theorem:iidResult} proves that this algorithm is at least 0.738-approximation for large enough number of items.

\begin{algorithm}
	\normalsize
	\caption{}
	\textbf{Input: $n$ iid items with distribution function $F$.}
	
	\begin{algorithmic}[1] \label{alg:iid}
		\STATE Set $a$ to 1.306 (root of $\cos(a)-\sin(a)/a-1$).
		\STATE Set $\theta_i=F^{-1}(\cos(ai/n)/\cos(a(i-1)/n))$.
		\STATE Pick the first item $i$ for which $X_i\geq \theta_i$.
	\end{algorithmic}
\end{algorithm}

\begin{theorem} \label{theorem:iidResult}
	For every $\epsilon>0$ there exists an $n_\epsilon$ such that for every $n\geq n_\epsilon$ Algorithm \ref{alg:iid} for $n$ items is at least $(1-\epsilon)\alpha$-approximation where $\alpha=1-\cos(a) \approx 0.7388$.
\end{theorem}

In the following we walk you through the steps of the design of Algorithm \ref{alg:iid} and provide a proof for Theorem \ref{theorem:iidResult}. For a given sequence of thresholds let $q_0,q_1,\ldots,q_n$ denote the probability of the algorithm not choosing any of the first items. More specifically, let $q_i=Pr[\tau>i]$ for every $0\leq i \leq n$. Knowing the thresholds $\theta_1,\ldots,\theta_n$ one can find this sequence by starting from $q_0=1$ and computing the rest using $q_{i}=q_{i-1} F(\theta_{i})$. Inversely, one can simply find the thresholds from $q_1,\ldots,q_n$ using $\theta_i=F^{-1}(q_i/q_{i-1})$. Hence, we focus the design of our algorithm on finding the sequence $q_1,\ldots,q_n$. To this end, we aim to find a continuous function $h:[0,1]\rightarrow[0,1]$ with $h(0)=1$ such that by setting $q_i=h(i/n)$ we can achieve our desired set of thresholds.

Note that such a function $h$ has to meet certain requirements. For instance, it has to be strictly decreasing, because at every step the algorithm picks an item with some positive probability, therefore $h(i/n)=q_i=Pr[\tau>i]$ is smaller for larger $i$. In the following we define a class of functions which has two additional properties. We prove that these properties can be useful in designing a useful threshold algorithm.

\begin{definition}
	A continuous and strictly decreasing function $h:[0,1]\rightarrow[0,1]$ with $h(0)=1$ is a threshold function if it has the following two properties:
	\begin{enumerate}[i.]
		\item $h$ is a strictly concave function.
		\item For every $\epsilon>0$ there exists some $\delta_0\leq \epsilon$ such that for every $\delta\leq\delta_0,\enspace\epsilon+\delta\leq s\leq 1$:$$\enspace h'(s-\delta)/h(s-\delta)\leq(1-\epsilon)h'(s)/h(s)\enspace .$$
	\end{enumerate}
\end{definition}

As shown in the following lemma, the first property leads to a decreasing sequence of thresholds. Also, we exploit the second property to show that the approximation factor of $h$ can be improved by increasing the number of items.

\begin{lemma} \label{lemma:decThresholds}
	If $h$ is a threshold function, then the sequence of thresholds $\theta_1,\ldots,\theta_n$ achieved from $h$ is decreasing.
\end{lemma}
\begin{proof}
	For every $1\leq i\leq n$ we have $\theta_i=F^{-1}(q_i/q_{i-1})$. Since every $q_i=h(i/n)$, we have $\theta_i=F^{-1}(\frac{h(i/n)}{h((i-1)/n)})$. Note that $F$ is a strictly increasing function, therefore having $\theta_i>\theta_{i+1}$ requires $\frac{h(i/n)}{h((i-1)/n)}>\frac{h((i+1)/n)}{h(i/n)}$. For simplicity let $x=i/n$ and $\delta=1/n$. From the first property of threshold functions we have:
	$$f(x) > \frac{f(x+\delta)+f(x-\delta)}{2}\enspace .$$
	By raising both sides to the power of 2, and subtracting $(f(x+\delta)/2-f(x-\delta)/2)^2$ from each side we have:
	\begin{align*}
		f(x)^2-\bigg(\frac{f(x+\delta)-f(x-\delta)}{2}\bigg)^2 &> \bigg(\frac{f(x+\delta)+f(x-\delta)}{2}\bigg)^2-\bigg(\frac{f(x+\delta)-f(x-\delta)}{2}\bigg)^2\\
		&=f(x+\delta)f(x-\delta)\enspace .
	\end{align*}	
	Therefore $f(x)^2 > f(x+\delta)f(x-\delta)$, which means $f(x)/f(x-\delta)>f(x+\delta)/f(x)$ and the proof is complete.
\end{proof}

In the following we define a class of functions, and prove for function of this class that its approximation factor approaches $\alpha$ for a large enough $n$. Doing so simplifies the job of finding a threshold function that results in an $\alpha$-approximation algorithm.

\begin{definition}
	A threshold function $h$ is $\alpha$-strong if it has the following properties:
	\begin{enumerate}[i.]
		\item $h(1)\leq 1-\alpha$.
		\item $\int_{0}^{1}h(r)dr\geq \alpha$.
		\item $\forall\enspace 0\leq s\leq 1:1-h(s)-h'(s)/h(s)\int_{s}^{1}h(r)dr\geq \alpha(1-\exp(h'(s)/h(s)))\enspace .$
	\end{enumerate}	
\end{definition}

The following theorem formally states the mentioned claim for $\alpha$-strong functions.

\begin{theorem} \label{Theorem:alphaStrong}
	If $h$ is an $\alpha$-strong function, then for every $\epsilon>0$ there exists an $n_\epsilon$ such that for every $n\geq n_\epsilon$ the threshold algorithm that acts based on $h$ is at least $(1-\epsilon)\alpha$-approximation on $n$ iid items.
\end{theorem}

\begin{proof}
	Let $OPT$ be a random variable that denotes the optimum solution and $ALG$ be a random variable that denotes the value picked by the algorithm. We can write the expectation of $OPT$ as
	\begin{align}
		E[OPT]=\int_{0}^{\infty}Pr[\max X_i\geq x]dx \enspace . \label{ineq:integralOpt}
	\end{align}
	Similarly the expectation of $ALG$ is
	\begin{align}
		E[ALG]=\int_{0}^{\infty}Pr[X_\tau\geq x]dx \enspace .\label{ineq:integralAlg}
	\end{align}
	The main idea behind the proof is to show for $\alpha$-strong functions that the integrand in \eqref{ineq:integralAlg} is an approximation of the integrand in \eqref{ineq:integralOpt} for every non-negative value of $x$. In particular, for every $\epsilon$ there exists some $n_\epsilon$ such that for every $n\geq n_\epsilon$ the second integrand is at least $(1-\epsilon)\alpha$ times the first integrand and this proves the theorem.
	
	Let us begin with finding an upper bound for the integrand in \eqref{ineq:integralOpt}. Let $G(x)=1-F(x)$ for every $x\in \mathcal{R}^{\geq 0}$. The following lemma gives an upper bound for $Pr[\max X_i\geq x]$ based on $G(x)$ and $n$.
	
	\begin{lemma} \label{lemma:OPTupperbound}
		For every $\epsilon>0$ there exists an $n_\epsilon$ such that for every $n\geq n_\epsilon$ the following inequality holds :$$Pr[\max X_i\geq x] \leq \frac{1-\exp(-nG(x))}{1-\epsilon}\enspace .$$
	\end{lemma}
	\begin{proof}
		For every $x\in\mathcal{R}^{\geq 0}$ we have:
		\begin{align}
			Pr[\max X_i\geq x] &= 1-F(x)^n \nonumber \\
			&= 1-(1-G(x))^n \nonumber \\
			&= 1-\bigg(\frac{1}{1-G(x)}\bigg)^{-n} \nonumber \\
			&= 1-\bigg(1+\frac{G(x)}{1-G(x)}\bigg)^{-n} \nonumber \\
			&\leq 1-\exp\bigg(\frac{-nG(x)}{1-G(x)}\bigg)\enspace .
		\end{align}
		We complete the proof by proving for every $\epsilon> 0$ that there exists an $n_\epsilon$ such that for every $n\geq n_\epsilon$ and $0\leq z\leq 1$, the ratio between $A(n,z)=1-\exp(-nz/(1-z))$ and $B(n, z)=1-\exp(-nz)$ is no more than $1/(1-\epsilon)$.
		
		For every $n$ and $z$ there are two cases:
		\begin{itemize}
			\item If $ln(n)/n\leq z\leq 1$ then we have:
			\begin{align}
				\frac{A(n,z)}{B(n,z)} \leq \frac{1}{B(n,z)} \leq \frac{1}{1-\exp(-ln(n))} = \frac{1}{1-1/n}\enspace .\label{ineq:nz1}
			\end{align}
			\item If $0\leq z\leq ln(n)/n$, we use partial derivatives of the functions to find an upper bound of their ratio. In the following the derivative of a function is with respect to variable $z$.
			\begin{align}
				\frac{A(n,z)}{B(n,z)}
				&= \frac{\int_{0}^{z}A'(n, w)dw}{\int_{0}^{z}B'(n, w)dw} \nonumber\\
				&= \frac{\int_{0}^{z}B'(n, w)\frac{A'(n, w)}{B'(n, w)}dw}{\int_{0}^{z}B'(n, w)dw} \nonumber\\
				&\leq \frac{\int_{0}^{z}B'(n, w)dw}{\int_{0}^{z}B'(n, w)dw}.\max_{0\leq w\leq z}\bigg\{\frac{A'(n, w)}{B'(n, w)}\bigg\} \nonumber\\
				&= \max_{0\leq w\leq z}\bigg\{\frac{A'(n, w)}{B'(n, w)}\bigg\} \nonumber\\
				&= \max_{0\leq w\leq z}\bigg\{\frac{n \exp(-nz/(1-z))/(1-z)^2}{n\exp(-nz)}\bigg\} \nonumber\\
				&= \max_{0\leq w\leq z}\bigg\{\frac{\exp(-nz^2/(1-z))}{(1-z)^2}\bigg\} \nonumber\\
				&\leq \frac{1}{(1-z)^2} \nonumber\\
				&\leq \frac{1}{1-2\ln(n)/n+ln^2(n)/n^2}\enspace . \label{ineq:nz2}
			\end{align}
		\end{itemize}
	Note that the denominators of both \eqref{ineq:nz1} and \eqref{ineq:nz2} become greater than $1-\epsilon$ as $n$ becomes greater than some $n_\epsilon$, thus the proof of the lemma follows.
	\end{proof}
	
	Lemma \ref{lemma:OPTupperbound} gives us an upper bound on $Pr[\max X_i\geq x]$. Now we aim to find a lower bound for $Pr[X_\tau\geq x]$. Through these two bounds we are able to find a lower bound on the approximation factor of the algorithm.
	
	In Lemma \ref{lemma:decThresholds} we showed that the thresholds are decreasing. Hence for an $x\in \mathcal{R}^{\geq 0}$, if $x<\theta_n$ then $Pr[X_\tau\geq x]$ is equal to $Pr[X_\tau\geq \theta_n]$ because the algorithm cannot pick an item below that value. Moreover, $Pr[X_\tau\geq \theta_n]$ is equal to $Pr[\tau\leq n]$ which is equal to $1-Pr[\tau>n]=1-q_n=1-h(1)$. The first property of $\alpha$-strong functions ensures that this number is at least $\alpha$. Since $Pr[\max X_i\geq x]$ is no more than 1, therefore, for every $x<\theta_n$ we have $Pr[X_\tau\geq x]\geq\alpha Pr[\max X_i\geq x]$.
	
	Now suppose $x\in \mathcal{R}^{\geq 0}$ and $x\geq \theta_n$. For $Pr[X_\tau\geq x]$ we have,
	\begin{align}
		Pr[X_\tau\geq x] &= \sum_{i=1}^{n}Pr[X_\tau\geq x|\tau=i]Pr[\tau=i] \nonumber \\
		&=\sum_{i=1}^{n}q_{i-1}(1-F(\max\{\theta_i,x\})) \enspace .\label{ineq:simpleProb} 
	\end{align}

	Since the thresholds are decreasing, there exists a unique index $j(x)$ for which $\theta_{j(x)}>x\geq\theta_{j(x)+1}$. For the sake of simplicity we assume there is an imaginary item $X_0$ for which $\theta_0=\infty$. In this way $j(x)$ is an integer number from 0 to $n-1$. By expanding \eqref{ineq:simpleProb} we have:
	\begin{align}
		Pr[X_\tau\geq x] &= \sum_{i=1}^{n}q_{i-1}(1-F(\max\{\theta_i,x\})) \nonumber \\
		&= \sum_{i=1}^{n}q_{i-1}G(\max\{\theta_i,x\}) \nonumber \\
		&=\sum_{i=1}^{j(x)}q_{i-1}G(\theta_i) + \sum_{i=j(x)+1}^{n}q_{i-1}G(x) \enspace . \label{ineq:expanded}
	\end{align}	
	
	The first sum in \eqref{ineq:expanded} is indeed the probability of picking one of the first $j(x)$ items, therefore we can rewrite it as $1-q_{j(x)}$. Hence,
	\begin{align}
		\Pr[X_\tau\geq x] &= 1-q_{j(x)}+\sum_{i=j(x)+1}^{n}q_{i-1}G(x) \nonumber \\
		&= 1-q_{j(x)} + n G(x)\sum_{i=j(x)+1}^{n}q_{i-1}\frac{1}{n} \nonumber \\
		&= 1-q_{j(x)} + n G(x)\sum_{i=j(x)+1}^{n}h((i-1)/n)\frac{1}{n} \nonumber \\
		&\geq 1-q_{j(x)} + n G(x)\int_{j(x)/n}^{1}h(r)dr \enspace . \label{ineq:riemann}
	\end{align}
	The integral in \eqref{ineq:riemann} comes from the fact that $h$ is a decreasing function and for such functions the Riemann sum of an interval is an upper bound of the integral of the function in that interval. For simplicity let $s(x)=j(x)/n$. Inequality \eqref{ineq:riemann} can be written as follows:
	\begin{align}
		Pr[X_\tau\geq x]\geq 1-h(s(x))+nG(x)\int_{s(x)}^{1}h(r)dr \enspace . \label{ineq:integralForm}
	\end{align}	
	
	In order to complete the proof of the theorem, we need to show that the right hand side of Inequality \eqref{ineq:integralForm} is an approximation of $Pr[\max X_i\geq x]$.
	
	\begin{lemma} \label{lemma:algLowerbound}
		For every $\epsilon>0$ there exists an $n_\epsilon$ such that for every integer $n\geq n_\epsilon$ the following inequality holds for every $x\geq \theta_n$:
		$$1-h(s(x))+nG(x)\int_{s(x)}^{1}h(r)dr\geq (1-\epsilon)\alpha(1-\exp(-nG(x)))\enspace .$$
	\end{lemma}
	\begin{proof}
		Recall that $s(x)=j(x)/n$ is a number from 0 to 1. We prove the correctness of the lemma by analyzing it for two different ranges of $s(x)$. For simplicity we may refer to $s(x)$ as $s$ in different parts of the proof. Suppose $s_0=min(0.5, \alpha)\epsilon$. For $0\leq s\leq s_0$ we have:
		\begin{align}
			1-h(s)+nG(x)\int_{s}^{1}h(r)dr
			&\geq nG(x)\int_{s}^{1}h(r)dr \nonumber \\
			&\geq nG(x)\int_{s_0}^{1}h(r)dr \nonumber \\
			&= nG(x)(\int_{0}^{1}h(r)dr-\int_{0}^{s_0}h(r)dr) \nonumber \\
			&\geq nG(x)(\int_{0}^{1}h(r)dr-s_0)	\label{ineq:simpleCase}\enspace.
		\end{align}
		From the second property of $\alpha$-strong functions we have $\int_{0}^{1}h(r)dr\geq \alpha$. Also, for every $z\in \mathcal{R}^{\geq 0}$ it holds that $z\geq 1-\exp(-z)$. By using these two inequalities in Inequality \eqref{ineq:simpleCase} the lemma is proved for this case:
		\begin{align*}
			1-h(s)+nG(x)\int_{s}^{1}h(r)dr
			&\geq nG(x)(\int_{0}^{1}h(r)dr-s_0) &\\
			&\geq (1-\exp(-nG(x)))(\alpha-s_0) \nonumber & \\
			&\geq (1-\exp(-nG(x)))\alpha(1-\frac{s_0}{\alpha})\nonumber\\
			&\geq (1-\exp(-nG(x)))\alpha(1-\epsilon)\nonumber & s_0\leq \alpha\epsilon
		\end{align*}
		Now what remains is the case that $s_0<s\leq 1$. Again, for this case we want the following inequality to hold:
		\begin{align}
			\frac{1-h(s)+nG(x)\int_{s}^{1}h(r)dr}{1-\exp(-nG(x))}\geq (1-\epsilon)\alpha\enspace . \label{ineq:mainIneq}
		\end{align}
		Recall that for every $x\geq \theta_n$, $s(x)=j(x)/n$ where $j(x)$ is the greatest index for which $\theta_j>x\geq \theta_{j+1}$. Since $G$ is a strictly decreasing function, we have $G(\theta_j)<G(x)\leq G(\theta_{j+1})$. Recall that for every $1\leq i\leq n$ we have $q_i=q_{i-1}(1-G(\theta_i))$, or equivalently $G(\theta_i)=1-q_i/q_{i-1}$. Therefore we can bound $G(x)$ as follows:
		\begin{align}
			1-q_j/q_{j-1} < G(x) \leq 1-q_{j+1}/q_j\enspace . \label{ineq:boundsGx}
		\end{align}
		Now, finding a lower bound for $1-q_j/q_{j-1}$ and an upper bound for $1-q_{j+1}/q_j$ in Inequality \eqref{ineq:boundsGx} gives us a lower bound and an upper bound for $G(x)$. For the lower bound we have
		$$G(\theta_j)=1-q_j/q_{j-1}=\frac{q_{j-1}-q_j}{q_{j-1}}=\frac{-(q_j-q_{j-1})}{q_{j-1}}=\frac{-(h(s)-h(s-1/n))}{h(s-1/n)} \enspace .$$
		By multiplying this fraction by $n/n$ we get:
		\begin{align}
			G(\theta_j)=\frac{-(\frac{h(s)-h(s-1/n)}{1/n})}{n\enspace h(s-1/n)}\geq \frac{-h'(s-1/n)}{n\enspace h(s-1/n)} \enspace , \label{ineq:derivative1}
		\end{align}
		where the last inequality in \eqref{ineq:derivative1} comes from the concavity of $h$. From the second property of threshold functions there exists some $\delta_0\leq s_0$ such that for every $n\geq 1/\delta_0, s_0+1/n\leq s\leq 1$ the following inequality holds:
		\begin{align}
			\frac{-h'(s-1/n)}{h(s-1/n)}\geq (1-s_0)\frac{-h'(s)}{h(s)}\enspace . \label{ineq:derivative2}
		\end{align}
		By using Inequality \eqref{ineq:derivative2} in Inequality \eqref{ineq:derivative1}, and by using that inequality in Inequality \eqref{ineq:boundsGx}, we get:
		\begin{align}
			G(x)>(1-s_0)\frac{-h'(s)}{n\enspace h(s)}\enspace . \label{ineq:lowerbound}
		\end{align}
		Similarly one can show the following upper bound on $G(x)$:
		\begin{align}
			G(x) &\leq G(\theta_{j+1}) & \nonumber \\
			&= 1-\frac{q_{j+1}}{q_{j}} & \nonumber \\
			&= \frac{-(h(s+1/n)-h(s))}{h(s)} & \nonumber \\
			&= \frac{-\frac{h(s+1/n)-h(s)}{1/n}}{n\enspace h(s)} & \text{multiplying by $\frac{n}{n}$} \nonumber \\
			&= \frac{-\frac{h(s+1/n)-h(s)}{1/n}}{n\enspace h(s+1/n)} & \text{since $h$ is decreasing} \nonumber \\
			&\leq \frac{-h'(s+1/n)}{n\enspace h(s+1/n)} \label{ineq:useful} & \text{concavity of $h$}\\
			&\leq \frac{1}{1-s_0}.\frac{-h'(s)}{n\enspace h(s)}\enspace. & \text{second property of threshold functions} \label{ineq:upperbound}
		\end{align}
		Using these bounds and the following auxiliary lemma we prove the correctness of Inequality \eqref{ineq:mainIneq}.
		\begin{lemma} \label{lemma:auxiliary}
			For every $z<0$ and $t\geq 1$ we have: $(1-\exp(zt))/(1-\exp(z))\leq t$.
		\end{lemma}
		\begin{proof}
			Let $A(z)=1-\exp(zt)$ and $B(z)=1-\exp(z)$. In the following the derivatives are with respect to $z$. For the ratio of these functions we have:
			\begin{align*}
				\frac{A(z)}{B(z)} &= \frac{\int_{0}^{z}A'(w)dw}{\int_{0}^{z}B'(w)dw} \\
				&=\frac{\int_{0}^{z}B'(w)\frac{A'(w)}{B'(w)}dw}{\int_{0}^{z}B'(w)dw}\\
				&\leq \max_{z\leq w\leq 0}\bigg\{\frac{A'(w)}{B'(w)}\bigg\}\frac{\int_{0}^{z}B'(w)dw}{\int_{0}^{z}B'(w)dw}\\
				&\leq \max_{z\leq w\leq 0}\bigg\{\frac{-t\exp(tw)}{-\exp(w)}\bigg\} \\
				&=\max_{z\leq w\leq 0}\bigg\{t\exp(w(t-1))\bigg\} \enspace .
			\end{align*}
			Since $w\leq 0$ and $t\geq 1$ the $\exp(w(t-1))\leq 1$, and the proof follows.
		\end{proof}
		By applying the bounds of Inequalities \eqref{ineq:lowerbound} and \eqref{ineq:upperbound} to the left hand side of Inequality \eqref{ineq:mainIneq} we have:
		\begin{align*}
			\frac{1-h(s)+nG(x)\int_{s}^{1}h(r)dr}{1-\exp(-nG(x))}
			&\geq \frac{1-h(s)-(1-s_0)h'(s)/h(s)\int_{s}^{1}h(r)dr}{1-\exp(-nG(x))} & \text{Inequality}\enspace \eqref{ineq:lowerbound}\\
			&\geq \frac{(1-s_0)(1-h(s)-h'(s)/h(s)\int_{s}^{1}h(r)dr)}{1-\exp(-nG(x))} & 1-h(s)\geq 0\\
			&\geq\frac{(1-s_0)(1-h(s)-h'(s)/h(s)\int_{s}^{1}h(r)dr)}{1-\exp(\frac{h'(s)}{h(s)(1-s_0)}))} & \text{Inequality}\enspace\eqref{ineq:upperbound} \enspace .
		\end{align*}
		By applying Lemma \ref{lemma:auxiliary} to the denominator we have:
		\begin{align*}
			\frac{1-h(s)+nG(x)\int_{s}^{1}h(r)dr}{1-\exp(-nG(x))}
			&\geq(1-s_0)^2.\frac{1-h(s)-h'(s)/h(s)\int_{s}^{1}h(r)dr}{1-\exp(h'(s)/h(s)))} \enspace .
		\end{align*}
		From the third property of $\alpha$-strong functions, the fraction at the right hand side of the above inequality is at least $\alpha$. Moreover, since $s_0\leq 0.5\epsilon$ it holds that $(1-s_0)^2\geq(1-\epsilon)$, and thus Inequality \eqref{ineq:mainIneq} holds and the proof of the lemma is complete.
	\end{proof}
	To wrap up the proof of the theorem we combine the results of the previous lemmas. Suppose $n_1$ and $n_2$ are the lower bounds of Lemma \ref{lemma:OPTupperbound} and Lemma \ref{lemma:algLowerbound} for $n$, respectively, such that their inequalities hold for $\epsilon/2$. For every $n\geq n_\epsilon = \max\{n_1,n_2\}$ we have:
	\begin{align}
	Pr[X_\tau\geq x]
	&\geq 1-h(s(x))+nG(x)\int_{s(x)}^{1}h(r)dr & \text{Inequality}\enspace \eqref{ineq:integralForm} \\
	&\geq (1-\epsilon/2)\alpha(1-\exp(-nG(x))) & \text{Lemma}\enspace  \ref{lemma:algLowerbound} \\
	&\geq (1-\epsilon/2)^2\alpha \enspace Pr[\max X_i\geq x] & \text{Lemma} \enspace\ref{lemma:OPTupperbound}\\
	&\geq (1-\epsilon)\alpha \enspace Pr[\max X_i\geq x] \enspace.\nonumber
	\end{align}
	This shows that for every non-negative value of $x$ the chance of the algorithm in picking an item with value at least $x$ is an approximation of the corresponding probability for the optimum solution. More specifically, we showed that for every $n\geq n_\epsilon$ and for every $x\geq 0$ the integrand of \eqref{ineq:integralAlg} is a $(1-\epsilon)\alpha$-approximation of the integrand of \eqref{ineq:integralOpt}, hence the theorem is proved.
\end{proof}

Now we have all the materials needed to prove Theorem \ref{theorem:iidResult}.

\begin{proof}[Proof of Theorem \ref{theorem:iidResult}]
	In order to prove the theorem, we demonstrate that the function $h(s)=\cos(as)$ is an $\alpha$-strong function, where $a\approx 1.306$ is a root of $\cos(a)+\sin(a)/a-1$ and $\alpha=1-\cos(a)$. To this end, we first need to show that this function is a threshold function:
	\begin{enumerate}[i.]
		\item To show the concavity of $h$ it suffices to show that its second derivative is negative for every $0<s\leq 1$. Note that $h'(s)=-a \sin(a s)$ and $h"(s)=-a^2\cos(a s)$.
		\item The ratio of $h'(s)/h(s)$ for every $s$ is equal to $-a\tan(a s)$. For every $\epsilon$ we need to show that there exists some $\delta_0\leq \epsilon$ such that for every $\delta\leq \delta_0$ and $\epsilon+\delta\leq s\leq 1$ the following holds:
		$$-a\tan(a (s-\delta)) \leq -(1-\epsilon)a\tan(a s)$$
		or equivalently, by dividing both sides to $-a$ and changing the direction of the inequality we want to have:
		$$\tan(a s-a \delta)) \geq (1-\epsilon)\tan(a s)\enspace .$$
		Note that $\tan(a s)$ is a convex function because $\tan"(a s)=2\tan(a s)\sec^2(a s)\geq 0$ for $0\leq s\leq 1$. For every $0\leq \delta\leq s$ in such functions we have:
		$$\frac{\tan(a s)-\tan(as-a\delta)}{a\delta}\leq \tan'(as)=\sec^2(as)\leq sec^2(a)\enspace .$$
		Therefore,
		$$\tan(a s)\leq \tan(as-a\delta)+a\delta\sec^2(a)\enspace .$$
		By multiplying both sides by $(1-\epsilon)$ and assuming that $\delta\leq\delta_0=\frac{\epsilon\tan(a\epsilon)}{a(1-\epsilon)\sec^2(a)}$ we have:
		\begin{align}
			(1-\epsilon)\tan(as) &\leq (1-\epsilon)(\tan(as-a\delta)+a\delta\sec^2(a)) \nonumber \\
			&\leq \tan(as-a\delta)-\epsilon\tan(as-a\delta)+(1-\epsilon)a\delta\sec^2(a) \nonumber \\
			&\leq \tan(as-a\delta)-\epsilon\tan(as-a\delta)+\epsilon\tan(a\epsilon) \nonumber \\
			&=\tan(as-a\delta)-\epsilon(\tan(a(s-\delta))-\tan(a\epsilon)) \label{ineq:2ndProperty}
		\end{align}
		Note that $\tan(x)$ is an increasing function, therefore for every $s\geq \epsilon+\delta$ Inequality \eqref{ineq:2ndProperty} is less than or equal to $\tan(as-a\delta)$, thus the second property holds as well.
	\end{enumerate}
	We showed that $h(s)=\cos(a s)$ is a threshold function. Now we prove that this threshold function is an $\alpha$-strong function too.
	Due to definition $\alpha=1-cos(a)=1-h(1)$, thus the first property holds. Moreover, $\int_{0}^{1}h(r)dr=sin(a)/a$. Again, due to definition $a$ is a root of $cos(a)+sin(a)/a-1$, and thus $sin(a)/a=1-cos(a)=\alpha$. Now we only need to show that the third property of $\alpha$-strong functions holds. To do so, we need to show that:
	\begin{align}
		1-\cos(as)+a\tan(as)[\sin(a)/a-\sin(as)/a]\geq\alpha(1-\exp(-a\tan(as)))\enspace . \label{ineq:finalIneq}
	\end{align} 
	By subtracting $\alpha(1-\exp(-a\tan(as)))$ from both sides and multiplying them by $\cos(a s)$ we have:
	$$\cos(a s)-\cos(as)^2+\sin(a)sin(as)-\sin(as)^2-\alpha\cos(as)+\alpha\cos(as)\exp(-a\tan(as)))\geq 0\enspace .$$
	Note that $\cos^2(as)+\sin^2(as)=1$, therefore the above inequality is equivalent to:
	$$(1-\alpha)\cos(as)+\sin(a)\sin(as)+\alpha\cos(as)\exp(-a\tan(as))\geq 1\enspace .$$
	Since $\sin(a)/a=1-\cos(a)=\alpha$ we can replace $\sin(a)$ with $\alpha a$. Also, from the relation between trigonometric functions we have $\cos(x)=1/\sqrt{1+\tan^2(x)}$ and $\sin(x)=\tan(x)/\sqrt{1+\tan^2(x)}$. By considering these equalities and assuming that $w=\tan(as)$ the above inequality becomes simplified as follows:
	$$\frac{1-\alpha}{\sqrt{1+w^2}}+\frac{\alpha a w}{\sqrt{1+w^2}}+\frac{\alpha \exp(-a w)}{\sqrt{1+w^2}}\geq 1\enspace .$$
	By multiplying both sides by $\sqrt{1+w^2}$ and raising them to the power of two, and subtracting $1+w^2$ from both sides we have:
	\begin{align*}
		(1-\alpha+\alpha a w + \alpha \exp(-a w))^2 - 1 - w^2 \geq 0
%		(1-\alpha)^2-1+2a\alpha(1-\alpha)w+((\alpha a)^2-1) w^2+\exp(-a w)(2 \alpha(1-\alpha)+2a\alpha^2 w+\alpha^2\exp(-a w))\geq 0
		\enspace .
	\end{align*}
	Suppose function $A(w)$ is the left hand side of the above inequality. To complete the proof we need to show that $A(w)$ is non-negative for every $0\leq w\leq \tan(a)$ because $w=\tan(as)$ and $0\leq s\leq 1$. First, let us take a look at the first three derivatives of $A(w)$ which are all continuous and bounded in range $[0,\tan(a)]$.
	
	\begin{align*}
		& A'(w)=2\alpha a (1-\exp(-a w))(1-\alpha+\alpha a w + \alpha \exp(-a w))-2w \\
		& A''(w)=2\alpha a^2 \exp(-aw)(1-3\alpha+\alpha a w + 2\alpha \exp(-aw))+2(\alpha^2 a^2-1) \\
		& A'''(w)=-2\alpha a^3\exp(-aw)(1-4\alpha+\alpha a w+4\alpha\exp(-aw))		
	\end{align*}
	
	In this part of the proof we frequently use one of the implications of intermediate value theorem: if $f(x)$ and $f'(x)$ are two continuous and bounded functions, then there exists a root of $f'(x)$ between every two roots of $f(x)$. This also implies that the number of the roots of $f(x)$ is at most one plus the number of the roots of $f'(x)$.
	
	We claim that $A'''(w)$ has at most two roots. The reason for this is because $-2\alpha a^3\exp(-aw)$ is always non-zero, and $1-4\alpha+\alpha a w+4\alpha\exp(-aw)$ has at most two roots, because its derivative, $\alpha a(1-4\exp(-aw))$ has exactly one root, which is $\ln(4)/a$. 
	
	The fact that $A'''(w)$ has at most two roots implies that $A''(w)$ has at most three roots, which are $w_1\approx 0.28157$, $w_2\approx 1.24251$, and $w_3\approx 2.27082$. We note that $A'(w)$ is positive at all these points. Therefore $A'(w)$ has at most two roots, because otherwise there would be a point in which $A'(w)\leq 0$ and $A''(w)=0$ which is impossible.
	
	Note that $A'(0)=0$, therefore $A'(w)$ has at most one root in $\mathcal{R}^+$. Now we note that $A(0^+)>0$ because $A'(0)=0$ and $A''(0)=2(\alpha a^2(1-\alpha)+\alpha^2 a^2-1)>0$. Also $A(\tan(a))>0$. Now if $A(w)<0$ for some $0<w<\tan(a)$, then $A(w)$ would have at least two roots in range $(0,\tan(a))$ which results in $A'(w)$ having two roots in $\mathcal{R}^+$. Since this is not true, we have $A(w)\geq 0$ for every $0\leq w\leq \tan(a)$.
	
	We proved that $A(w)$ is non-negative in $[0,\tan(a)]$, therefore Inequality \eqref{ineq:finalIneq} holds for every $0\leq s\leq 1$. This means that $h(s)=\cos(as)$ has all three properties of an $\alpha$-strong function for $\alpha\approx0.7388$.
 %	This \href[options]{https://www.wolframalpha.com/input/?i=Plot%5B(1-cos(1.306542374+x)%2B((sin(1.306542374)-sin(1.306542374+x))+tan(1.306542374+x)))%2F(1-e%5E(-1.306542374+tan(1.306542374+x))),+%7Bx,+0,+1%7D%5D}{WolframAlpha link} ensures that this always holds. If we prove it theoretically, then we are all done! :-)
%	\todo{Worst case scenario is to use high order polynomial lower bounds and upper bounds, but we'd like to be clean!}
\end{proof}


==> old_notes/large_market.tex <==
In this section we study more generalized cases of the prophet inequalities problem. Suppose $X_1,\ldots,X_n$ are random variables from distribution functions $F_1,\ldots,F_n$. Similar to Section \ref{section:iid} we assume, for the sake of simplicity, that all distribution functions are continuous and strictly increasing on a subinterval of $\mathcal{R}^+$. The goal of this section is to show improving results for the best order, random orders, and arbitrary orders of \textit{large market} instances. We use the term large market as a general term to refer to instances with repeated distributions. The following definition formally captures this concept.

\begin{definition}
	A set of $n$ items with distribution functions $F_1,\ldots,F_n$ is $m$-frequent if for every item in this set there are at least $m-1$ other items with the same distribution function.
\end{definition}

In the remainder of this section we show for the best order and a random order of a large market instance that one can find a sequence of thresholds which in expectation performs as good as our algorithm for iid items. Roughly speaking, we design algorithms that are $\alpha$-approximation for large enough $m$-frequent instances, where $\alpha\approx 0.7388$. The following two theorems formally state our results for the best order and a random order, respectively.
 
\begin{theorem}\label{theorem:bestOrder}
	For every $\epsilon>0$ and set $\mathbb{X}$ of $n$ items, there exists $m_\epsilon$ such that if $\mathbb{X}$ is $m$-frequent for $m\geq m_\epsilon$ then there exits an algorithm which is $(1-\epsilon)\alpha$-approximation on a permutation of $\mathbb{X}$.
\end{theorem}

\begin{theorem}\label{theorem:randOrder}
	For every $\epsilon>0$ and set $\mathbb{X}$ of $n$ items there exists $c_\epsilon$ such that if $\mathbb{X}$ is $m$-frequent for $m\geq c_\epsilon \log(n)$ then there exists an algorithm which in expectation is $(1-\epsilon)\alpha$-approximation on a random permutation of $\mathbb{X}$.
\end{theorem}

To prove the theorems we first provide an algorithm for a specific class of large market instances, namely partitioned sequences. Lemma \ref{lemma:partition} states that this algorithm is $\alpha$-approximation when the number of partitions is large. We later show how to apply this algorithm on the best order an a random order of large market instances a achieve a similar approximation factor. The formal definition of partitioned sequences is in the following.

\begin{definition}
	A sequence of items with distribution functions $F_1,\ldots,F_n$ is $m$-partitioned if $n=mk$ and the sequence of functions $F_{ik+1},\ldots,F_{ik+k}$ is a permutation of $F_1,\ldots,F_k$ for every $0\leq i<m$.
\end{definition}

The following algorithm exploits Algorithm \ref{alg:iid} for iid items in order to find thresholds for a partitioned large market instance. 

\begin{algorithm}
	\normalsize
	\caption{}
	\textbf{Input: An $m$-partitioned sequence of items with distribution functions $F_1,\ldots,F_n$.}
	
	\begin{algorithmic}[1] \label{alg:largeMarket}
		\STATE Let $k=n/m$.
		\STATE Let $F(x)=\prod_{i=1}^{k}F_i(x)$.
		\STATE Let $\theta_1\ldots,\theta_m$ be the thresholds by Algorithm \ref{alg:iid} for $m$ iid items with distribution function $F$.
		\STATE Pick the first item $i$ if $X_i\geq \theta_{\lceil i/k \rceil}$.
	\end{algorithmic}
\end{algorithm}

\begin{lemma} \label{lemma:partition}
	For every $\epsilon>0$ there exists an $m_\epsilon$ such that for every $m\geq m_\epsilon$ Algorithm \ref{alg:largeMarket} is $(1-\epsilon)\alpha$-approximation on an $m$-partitioned input.
\end{lemma}

\begin{proof}
	Let $X_1,\ldots,X_n$ be random variables representing the items, and let $Y_1,\ldots,Y_m$ be iid random variables with distribution function $F(x)=\prod_{i=1}^{k}F_i(x)$. For the expectation of the maximum of these variables we have:
	\begin{align}
		E[\max_{i=1}^{k} Y_i]
		&= \int_{0}^{\infty} Pr[\max_{i=1}^{k} Y_i\geq x] dx \nonumber \\
		&= \int_{0}^{\infty} \bigg(1-\prod_{i=1}^{m}F(x)\bigg) dx \nonumber \\
		&= \int_{0}^{\infty} \bigg(1-\prod_{i=1}^{m}\prod_{j=1}^{k}F_j(x)\bigg) dx \nonumber \\
		&= \int_{0}^{\infty} \bigg(1-\prod_{i=1}^{n}F_i(x)\bigg) dx \nonumber \\
		&= \int_{0}^{\infty} Pr[\max_{i=1}^{n} X_i\geq x] dx \nonumber \\
		&= E[\max_{i=1}^{n}X_i] \label{ineq:optsAreEq}
	\end{align}
	This shows that the optimum solution is the same for both sets of items. Let $\tau_Y$ and $\tau_X$ be random variables that denotes the index of the picked items in $Y_1,\ldots,Y_m$ and $X_1\ldots,X_n$ respectively. Theorem \ref{theorem:iidResult} states that there exists some $s$ such for every $m\geq s$, we have $E[Y_{\tau_Y}] \geq (1-\epsilon/2)\alpha E[\max_{i=1}^{m}Y_i]$. In the following we show that there exist some $m_2$ such that for every $m\geq m_2$, $E[X_{\tau_X}]\geq (1-\epsilon/2)E[Y_{\tau_Y}]$. This proves the lemma for every $m\geq m_\epsilon=\max\{s,m_2\}$, i.e.
	$$E[X_{\tau_X}]\geq (1-\epsilon/2)E[Y_{\tau_Y}]\geq (1-\epsilon/2)^2\alpha E[\max_{i=1}^{m}Y_i]\geq (1-\epsilon)\alpha E[\max_{i=1}^{m}Y_i]=(1-\epsilon)\alpha E[\max_{i=1}^{n}X_i]\enspace .$$
	
	Since for every non-negative random variable $Z$, $E[Z]=\int_{0}^{\infty}Pr[Z\geq z]dz$, therefore, in order to show $E[X_{\tau_X}]\geq (1-\epsilon/2)E[Y_{\tau_Y}]$ we show $Pr[X_{\tau_X}]\geq(1-\epsilon/2) Pr[Y_{\tau_Y}]$ for every $x\geq 0$.
	
	In the following, we use $G_i(x)$ to denote $1-F_i(x)$. For every non-negative $x$ we have:
	\begin{align}
		Pr[X_{\tau_X}\geq x]
		&= \sum_{i=1}^{n}Pr[X_{\tau_X}\geq x|\tau_X=i]Pr[\tau_X=i] \nonumber \\
		&= \sum_{i=1}^{n}\prod_{j=1}^{i-1}F_j(\theta_{\lceil j/k \rceil}) G_i(\max\{x,\theta_{\lceil i/k \rceil}\})\nonumber
	\end{align}
	By rewriting the above sum with respect to the $m$ partitions we have:
	\begin{align}
		Pr[X_{\tau_X}\geq x]
		&= \sum_{i=0}^{m-1}\sum_{j=1}^{k}\prod_{l=1}^{ik+j-1}F_l(\theta_{\lceil l/k\rceil})G_{ik+j}(\max\{x,\theta_{i+1}\}) \nonumber \\
		&= \sum_{i=0}^{m-1}\sum_{j=1}^{k}\bigg(\prod_{l=1}^{ik}F_l(\theta_{\lceil l/k\rceil})\prod_{p=1}^{j-1}F_{ik+p}(\theta_{i+1})G_{ik+j}(\max\{x,\theta_{i+1}\})\bigg) \nonumber \\
		&= \sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{ik}F_l(\theta_{\lceil l/k\rceil})\sum_{j=1}^{k}\prod_{p=1}^{j-1}F_{ik+p}(\theta_{i+1})G_{ik+j}(\max\{x,\theta_{i+1}\}) \bigg ) \enspace . \label{ineq:messy}
	\end{align}
	
	Note that $X_1,\ldots,X_n$ are $m$-partitioned, hence for every partition $0\leq i< m$ and $x\geq 0$ we have $\prod_{l=ik+1}^{ik+k}F_l(x)=F(x)$. Therefore $\prod_{l=1}^{ik}F_l(\theta_{\lceil l/k\rceil})=\prod_{l=1}^{i}F(\theta_{l})$. By this replacement, Inequality \eqref{ineq:messy} can be written as follows:
	\begin{align}
	Pr[X_{\tau_X}\geq x]
	&= \sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}\prod_{p=1}^{j-1}F_{ik+p}(\theta_{i+1})G_{ik+j}(\max\{x,\theta_{i+1}\}) \bigg ) \enspace . \label{ineq:messy2}
	\end{align}
	
	Moreover, for every $0\leq i<m$ and $1\leq j\leq k$ we have:
	\begin{align}
		\prod_{p=1}^{j-1}F_{ik+p}(\theta_{i+1})
		&\geq \prod_{p=1}^{k}F_{ik+p}(\theta_{i+1}) & Every\enspace F_t(x)\enspace is\enspace at\enspace most\enspace 1\nonumber \\
		&= F(\theta_{i+1}) & \nonumber \\
		&= 1-G(\theta_{i+1}) & \nonumber \\
		&\geq 1-\frac{a\tan(a)}{m} & Inequality\enspace \ref{ineq:useful} \enspace for \enspace h(s)=\cos(as) \enspace. \nonumber \\
		&\geq 1-\epsilon/2 & For\enspace every \enspace m\geq m_2= \frac{2a\tan(a)}{\epsilon}\label{ineq:prodSimple}
	\end{align}
	
	Inequality \eqref{ineq:prodSimple} shows that for a large enough $m$, the left hand side of the inequality becomes close enough to 1. By using this inequality in Inequality \eqref{ineq:messy2} we have:
	\begin{align}
		Pr[X_{\tau_X}\geq x] &\geq \sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}(1-\epsilon/2)G_{ik+j}(\max\{x,\theta_{i+1}\}) \bigg ) \nonumber \\
		&= (1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}G_{ik+j}(\max\{x,\theta_{i+1}\}) \bigg ) \label{ineq:messy3} \enspace .
	\end{align}
	
	Let $r=\max\{x, \theta_{j+1}\}$. By multiplying every term in Inequality \eqref{ineq:messy3} by $\prod_{p=1}^{j-1}F_{ik+p}(r)$, which is less than or equal to 1, we have:	
	\begin{align}
	Pr[X_{\tau_X}\geq x]
	&\geq (1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}G_{ik+j}(r) \bigg ) & \nonumber \\ 
	&\geq (1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}\prod_{p=1}^{j-1}F_{ik+p}(r)G_{ik+j}(r) \bigg )& \nonumber \\
	&=	(1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}\prod_{p=1}^{j-1}F_{ik+p}(r)(1-F_{ik+j}(r)) \bigg ) & \nonumber \\
	&=	(1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\sum_{j=1}^{k}\bigg(\prod_{p=1}^{j-1}F_{ik+p}(r)-\prod_{p=1}^{j}F_{ik+p}(r)\bigg) \bigg ) & \nonumber \\
	&=	(1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\bigg(1-\prod_{p=1}^{k}F_{ik+p}(r)\bigg) \bigg ) & \text{Telescoping series} \nonumber \\
	&=	(1-\epsilon/2)\sum_{i=0}^{m-1}\bigg(\prod_{l=1}^{i}F(\theta_l)\bigg(1-F(r)\bigg) \bigg ) & \nonumber \\
	&= (1-\epsilon/2)\sum_{i=0}^{m-1}\prod_{l=1}^{i}F(\theta_l)G(r) \enspace . & \label{ineq:messy4}
	\end{align}
	
	Note that $Pr[Y_{\tau_Y}\geq x]=\sum_{i=0}^{m-1}\prod_{l=1}^{i}F(\theta_l)G(\max\{x,\theta_{i+1}\})$. Using this in Inequality \eqref{ineq:messy4} results that $Pr[X_{\tau_X}\geq x]\geq (1-\epsilon/2)Pr[Y_{\tau_Y}\geq x]$, hence the proof is complete.
\end{proof}

\begin{proofof} [Theorem \ref{theorem:bestOrder}]
	Let $s$ be the lower bound on the number of partitions in Lemma \ref{lemma:partition} for $\epsilon/2$, and let $m_\epsilon=2(s-1)/\epsilon$. The outline of the proof is as follows. Let $\mathbb{X}$ be an $m$-frequent set of items for $m\geq m_\epsilon$. We uniformly group the items into $s$ parts with $\lfloor m/s \rfloor$ items of each type in every group. Let $\mathbb{Y}$ denote the set of partitioned items. In order to make all parts similar, we may need to discard some of the items, however, we show this does not hurt the approximation factor significantly. Finally, by applying Algorithm \ref{alg:largeMarket} to $\mathbb{Y}$ we achieve the desired approximation factor.
	
	The following lemma shows that discarding a fraction of items influences the approximation factor proportionally.
	\begin{lemma} \label{lemma:discard}
		Let $\{X_1,\ldots,X_n\}$ be a $k$-frequent set of items. Suppose for some $S\subseteq\{1,\ldots,n\}$ that the set $\{X_{S_1},\ldots,X_{S_r}\}$ is $p$-frequent and contains every $X_i$ for $1\leq i\leq n$. Then we have
		$$E[\max_{i\in S}X_i] \geq \frac{p}{k}E[\max_{1\leq i\leq n}X_i] \enspace .$$
	\end{lemma}
	\begin{proof}
		Let $\rho$ and $\rho'$ be random variables that denote the index of the maximum with the smallest index amongst $X_1,\ldots,X_n$ and $X_{S_1},\ldots,X_{S_r}$, respectively. Then,
		\begin{align*}
			E[\max_{i\in S}X_i]
			&= \sum_{i\in S}E[X_i|i=\rho']Pr[i=\rho'] \\
			&\geq \sum_{i\in S}E[X_i|i=\rho]Pr[i=\rho] \\
			&\geq \frac{p}{k}\sum_{i=1}^{n}E[X_i|i=\rho]Pr[i=\rho] \\
			&= \frac{p}{k}E[\max_{1\leq i\leq n}X_i] \enspace.
		\end{align*}
		Therefore, the proof is complete.
	\end{proof}
	
	Note that in partitioning $\mathbb{X}$ to $s$ groups there might be at most $s-1$ items of each type being discarded in $\mathbb{Y}$, therefore $\mathbb{Y}$ is $(m-s+1)$-frequent. Let $ALG$ be a random variable that denotes the value of the item picked by our algorithm. We have:
	\begin{align*}
		E[ALG] &\geq (1-\epsilon/2)\alpha E[\max_{Y\in\mathbb{Y}}Y] & \text{Lemma} \enspace \ref{lemma:partition} \\
		&\geq (1-\epsilon/2)\alpha \frac{m-s+1}{m}E[\max_{X\in\mathbb{X}}X] & \text{Lemma} \enspace \ref{lemma:discard} \\
		&\geq (1-\epsilon/2)^2\alpha E[\max_{X\in\mathbb{X}}X] & \\
		&\geq (1-\epsilon)\alpha E[\max_{X\in\mathbb{X}}X] \enspace .
	\end{align*}
	Therefore, for every $m$-frequent set $\mathbb{X}$ there exists an ordering of its items  on which our algorithm is $(1-\epsilon)\alpha$-approximation.
\end{proofof}

\begin{proofof} [Theorem \ref{theorem:randOrder}]
	Let $\pi$ be a random permutation of the items. Consider $s$ different partitions for the items, i.e. one from $X_{\pi_1}$ to $X_{\pi_{n/s}}$, one from $X_{\pi_{n/s+1}}$ to $X_{\pi_{2 n/s}}$, so on so forth. We show that when the number of similar items is large enough then a random permutation is very likely to uniformly distribute similar items into these parts. Therefore, by discarding a small fraction of the items $X_{\pi_1},\ldots,X_{\pi_n}$ can be assumed as an $s$-partitioned sequence, hence Algorithm \ref{alg:largeMarket} can be applied to it.
	
	Note that $\mathbb{X}$ is $m$-frequent, which means that for every item $i$ there are at least $m-1$ other items with the same distribution functions as $F_i$. We refer to a set of similar items as a type. Therefore, there are at least $m$ items of every type in $\mathbb{X}$. We use the following lemma to show for every type that with a high probability the number of items of that type in every partition is almost $m/s$.
	
	\begin{lemma} [\cite{panconesi1997randomized}] \label{lemma:chernoff}
		Let $x_1,\ldots,x_m$ be a sequence of negatively correlated boolean (i.e. 0 or 1) random variables, and let $X=\sum_{i=1}^{m} x_i$. We have:
		$$Pr[|X-E[X]|\geq \delta E[X]] \leq 3\exp(-\delta^2E[X]/3)\enspace .$$
	\end{lemma}
	
	Since $\pi$ is a random permutation, the expected number of these items in a fixed partition is $m/s$. Using Lemma \ref{lemma:chernoff}, with probability at most $3\exp(\frac{-\delta^2 m}{3 s})$ there are less than $(1-\delta)m/s$ of these items in a fixed partition. Using Union Bound on all the $s$ partitions and all types of items (note that there at at most $n/m$ types), with probability at most $3 s \frac{n}{m}\exp(\frac{-\delta^2 m}{3 s})$ there is a type of item  which has less than $(1-\delta)m/s$ items in a partitions. If we choose $\delta=\epsilon/3$ then for every $m\geq \frac{3 s}{\delta^2}(\log(n)+\log(\frac{9}{\epsilon}))$ this probability becomes less than $\epsilon/3$.
	%Note that $s$, $\epsilon$, and $\delta$ are all constants.
	
	Now we are ready to wrap up the proof. If we choose $s=m_{\epsilon/3}$ using Lemma \ref{lemma:partition}, $\delta=\epsilon/3$, and $c_\epsilon=\frac{3s\log(9/\epsilon)}{\delta^2}$ then for every $m\geq c_\epsilon\log(n)$ with probability at least $(1-\epsilon/3)$ there are at least $(1-\epsilon/3)m/s$ items of each type in every partitions. In such cases by discarding at most $\epsilon/3$ fraction of the items of each type we have exactly $(1-\epsilon/3)m/s$ of them in each partition. Lemma \ref{lemma:discard} states that removing this fraction of items changes the approximation factor by at most $(1-\epsilon/3)$. This means that for a random permutation of the items, with probability at least $(1-\epsilon/3)$ we can loose on the approximation factor by no worse than $(1-\epsilon/3)$ and have an $s$-partitioned sequence. Due to Lemma \ref{lemma:partition}, Algorithm \ref{alg:largeMarket} is $(1-\epsilon/3)\alpha$-approximation on this number of partitions. Therefore, the approximation factor of our method is $(1-\epsilon/3)^3\alpha$ which is more than $(1-\epsilon)\alpha$.
\end{proofof}


==> old_notes/large_market_old_notes.tex <==
Let $A=\langle A_1, \ldots, A_n \rangle$ be a given sequence of distributions for which every $A_i$ comes from a set of distribution types $T=\{T_1, \ldots, T_m\}$. The frequency $f_i(A)$ of each distribution type $T_i$ in $A$ is defined as the number of times $T_i$ appears in $A$. The \textit{large market} assumption the assumption is that every distribution type appears in $A$ for at least $k$ times, i.e. $\min\{f_i(A)\}\geq k$ for some integer $k$. The highest $k$ here specifies $f(A)$, the frequency of $A$.

So far in this paper, we have proposed an algorithm for the \textit{i.i.d.} setting that has a 0.74-competitive ratio. For more general cases $A$, the sequence of distributions, may contain two or more different types of distributions. But does this devalue our algorithm? The large market setting considers more general cases of the Prophet Inequality problem in which a variety of distribution types appear in $A$. In this section we exploit our algorithm for the \textit{i.i.d.} setting in order to design algorithms for the large market setting. For each of the best order \ref{subsection:best_order} and the random order \ref{subsection:random_order} problems the competitive ratios of our algorithms are directly related to the number of times every distribution type appears in $A$, i.e. the higher the frequency of $A$, the better the competitive ratios of our algorithms. 

\subsection{Best Order} \label{subsection:best_order}
\input{best_order.tex}
\subsection{Random Order} \label{subsection:random_order}
%\input{random_order.tex}



==> old_notes/melika.tex <==


%\section{Prophet Inequality for Random Variables with i.i.d Distributions}

Let $X_1, X_2, \dots , X_n$ be i.i.d random variables with common distribution function $\mathcal{F}$, where $\mathcal{F}$ is assumed to be continuous and non-decreasing. A prophet who can see all the sampled values and choose the maximum will obtain an expected profit of $E(\max\limits_{1 \leq j \leq n} X_i)$. The gambler, on the other hand, observes the sequence $X_1, X_2, \dots, X_n$ one at a time, and can stop the sequence at any time to collect the most recent reward. The rest of the sequence will not be revealed to him once he requests a stop. If the gambler picks a single threshold, and picks the first sample which exceeds this threshold as his prize, $1-\frac{1}{e}$ is the best approximation factor he can hope for. In this section, we present an algorithm that beats this approximation factor. 

Let $\theta_1,\theta_2,\dots ,\theta_n$ be fixed constants determined later. Consider the algorithm in which the gambler chooses the first sample $X_k$ such that $X_k \ge \theta_k$. Let $\tau$ denote the index of the sample at which the gambler stops the sequence and picks the prize using our algorithm. The expected profit of the gambler would be 
$$E(X_{\tau}) = \int_{0}^{\infty}{Pr(X_{\tau} > t) dt}$$
As we mentioned earlier, the prophet can simply pick the maximum of $X_i$'s and so he makes an expected profit of $$E(\max\limits_{1 \leq j \leq n} X_i) = \int_{0}^{\infty}{Pr(\max\limits_{1 \leq j \leq n} X_i > t)}$$
If we compare the integrands and show that $Pr(X_{\tau} > t) \ge \alpha Pr(\max\limits_{1 \leq j \leq n} X_i > t)$ for a constant $\alpha \in \mathit{R}^{+}$ and every $t \ge 0$, then our proposed algorithm is an $\alpha$-approximation for the gambler. We can write $Pr(X_{\tau} > t)$ as the following summation.
$$Pr(X_{\tau} > t) = \sum_{i=1}^n{Pr(\tau = i ~~\textit{and}~~ X_{\tau} > t)} $$

Let $p_i$ denote the probability that the gambler stops the sequence before $X_i$. For any index $i$, the event that the gambler picks $X_i$ and also $X_i$ is bigger than $t$ happens exactly when the gambler does not terminate the sequence before arriving at $X_i$ and also $X_i$ is bigger than both $\theta_i$ and $t$. Therefore, the probability of this event would be $(1-p_i)(1-F(\max\{t,\theta_i\})$. Hence, we have

$$Pr(X_{\tau} > t) = \sum_{i=1}^n{(1-p_i)(1-F(\max\{t,\theta_i\}))}$$

Let $G(t)$ denote $1-F(t)$ for any real number $t$. Then
$$Pr(X_{\tau} > t) = \sum_{i=1}^n{(1-p_i)\min\{G(t),G(\theta_i)\}}$$

Note that we have not yet determined the threshold values. Suppose we can set $\theta_i$'s in a way that we have $\theta_i = G^{-1}(\frac{p_{i+1}-p_i}{1-p_i})$ for any index $i$. Then $G(\theta_i) = \frac{p_{i+1}-p_i}{1-p_i}$ which is exactly equal to the probability that the gambler stops the sequence at $X_i$ given that he has not stopped the sequence before $X_i$. As the gambler advances through the sequence, the probability that he picks the most recently revealed random variable increases. Thus, $G(\theta_i)$ would increase as $i$ increases. For a fixed $t$, let $j$ denote the largest index such that $G(t) \le G(\theta_j)$. Then we can simplify the above equation as 

\begin{multline*}\nonumber
%\begin{split}
Pr(X_{\tau} > t) = \sum_{i=1}^n{(1-p_i)\min\{G(t),G(\theta_i)\}} \\\nonumber=  \sum_{i=1}^j{(1-p_i)~G(\theta_i)} + G(t) \sum_{i=j+1}^n{(1-p_i)} =  p_{j+1} + G(t) \sum_{i=j+1}^n{(1-p_i)}
%\end{split}
\end{multline*}

where the last equation follows from definition of $\theta_i$'s.
Recall that our goal is to show $Pr(X_{\tau} > t) \ge \alpha Pr(\max\limits_{1 \leq j \leq n} X_i > t)$ for the maximum possible constant $\alpha$ and our choice of threshold values. The right hand side probability is equal to $1-F(t)^n$. Thus now it suffices to find $\alpha$ and set the thresholds such that $$p_{j+1} + G(t) \sum_{i=j+1}^n{(1-p_i)} \ge \alpha (1-F(t)^n).$$ 


Let $h$ be a continuous function on domain $[0,1]$ such that $h(\frac{i}{n}) = 1-p_i$ for any index $i \in [n]$. By substituting $p_i$ with $1-h(\frac{i}{n})$ for each index $i$ in the above inequality we will have

$$1-h(\frac{j+1}{n}) + G(t) \sum_{i=j+1}^n{h(\frac{i}{n})} \ge \alpha (1-F(t)^n)$$

or equivalently, 
\begin{equation}\label{p1}
1-h(\frac{j+1}{n}) + nG(t) \sum_{i=j+1}^n{\frac{1}{n}h(\frac{i}{n})} \ge \alpha  (1-F(t)^n)
\end{equation}

Fix $n$ and $t$ and let $\phi = nG(t)$. The right hand side of the above inequality can be rewritten as $\alpha(1-(1-\frac{\phi}{n})^n)$. For large values of $n$, the right hand side would approach $\alpha(1-e^{-\phi})$, and the summation on the left hand side can be rewritten as an integral. Our approach would be to find function $h$ and maximum constant $\alpha$ so that the inequality 

$$1-h(s) + \phi \int_{\tau=s}^1{h(\tau)d{\tau}} \ge \alpha  (1-e^{-\phi})$$

is satisfied for any $s \in [0,1]$ and any $\phi > 0$. Then we would have the probability $p_i$ from the equation $p_i = 1-h(\frac{i}{n})$ for each index $i$. Furthermore, the thresholds can be set by the previously mentioned relation $\theta_i = G^{-1}(\frac{p_{i+1}-p_i}{1-p_i})$ so that Inequality \ref{p1} is satisfied yielding an $\alpha$-approximation algorithm.

\begin{comment}
\begin{lemma}
$Pr(\tau = k) = \frac{1}{n}$ for every $k \in {1,2,\dots,n}$. 
\end{lemma}

\begin{proof}
\begin{eqnarray}
Pr(\tau = k) = Pr(X_k \ge \theta_k) \prod\limits_{i=1}^{k-1} {Pr(X_i < \theta_i)}  = (1-F(\theta_k))\prod\limits_{i=1}^{k-1}{ F(\theta_i)}  
\end{eqnarray}
By definition of $\theta_i$, we have $F(\theta_i) = \frac{n-i}{n-i+1}$. Therefore,

\begin{eqnarray}
(1-F(\theta_k))\prod\limits_{i=1}^{k-1}{ F(\theta_i)} = \frac{1}{n-k+1} \prod\limits_{i=1}^{k-1}{ \frac{n-i}{n-i+1}} = \frac{1}{n} 
\end{eqnarray}\qedsymbol
\end{proof}
\end{comment}




